Examining Cross-lingual Contextual Embeddings with Orthogonal Structural Probes

State-of-the-art contextual embeddings are obtained from large language models available only for a few languages. For others, we need to learn representations using a multilingual model. There is an ongoing debate on whether multilingual embeddings can be aligned in a space shared across many languages. The novel Orthogonal Structural Probe (Limisiewicz and Mare\v{c}ek, 2021) allows us to answer this question for specific linguistic features and learn a projection based only on mono-lingual annotated datasets. We evaluate syntactic (UD) and lexical (WordNet) structural information encoded inmBERT's contextual representations for nine diverse languages. We observe that for languages closely related to English, no transformation is needed. The evaluated information is encoded in a shared cross-lingual embedding space. For other languages, it is beneficial to apply orthogonal transformation learned separately for each language. We successfully apply our findings to zero-shot and few-shot cross-lingual parsing.

==> sections/old.tex <==
% \begin{table*}[!ht]
% \centering
% \scriptsize
% \begin{tabular}{@{}l|ccccccccc|ccccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c|}{\textbf{Dependency Distance Spearman's Correlation}} & \multicolumn{9}{c}{\textbf{UUAS}} \\
% & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU}
% & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
% \textsc{Distinct} & .813 & .859 & .857 & .838 &  .829 &  &  &  & -
% &  &  &  &  &  &  &  &  &  - \\
% \citet{chi2020finding} & .817 & .859 & - & .807 &  .777 &  &  &  & -
% & 80.1 & 79.4 & - & 74.4 & 66.3 &  &  &  & - \\ \midrule
% \textsc{Mapped} & .811 & .858 & .857 & .839 & .828 &  &  &  &
% &  &  &  &  &  &  &  &  & \\ \midrule
% \textsc{Same} &  .813 & .849 & .850 & .828 &  .799 &  &  & &
% &  &  &  &  &  &  &  &  & \\ 
% \citet{chi2020finding} & .806 & .848 & - & .789  &  .717 &  &  & & - 
% & 75.9 & 77.6 & - &  73.1 & 57.8 &  &  & & - \\ \midrule
% \end{tabular}
% \caption{Results on dependency structure correlation and Undirected Unlabeled Attachement Score. Compared with \emph{Standard Structural Probes} after \citet{chi2020finding}.}
% \label{tab:dependency-distance-results}
% \end{table*}


% \begin{table*}[!ht]
% \centering
% \scriptsize
% \begin{tabular}{@{}l|ccccccccc|ccccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c|}{\textbf{Dependency Depth Spearman's Correlation}} & \multicolumn{9}{c}{\textbf{UAS}} \\
% & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU}
% & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
% \textsc{Distinct} & .813 & .859 & .857 & .838 &  .829 &  &  &  & -
% &  &  &  &  &  &  &  &  &  - \\ \midrule
% \textsc{Mapped} & .811 & .858 & .857 & .839 & .828 &  &  &  &
% &  &  &  &  &  &  &  &  & \\ \midrule
% \textsc{Same} &  .813 & .849 & .850 & .828 &  .799 &  &  & &
% &  &  &  &  &  &  &  &  & \\  \midrule
% \end{tabular}
% \caption{Results on dependency structure correlation and nlabeled Attachement Score}
% \label{tab:dependency-depth-results}
% \end{table*}


% \begin{table*}[!ht]
% \centering
% \tiny
% \begin{tabular}{@{}l|ccccccccc|ccccccccc@{}}
% \toprule
% \multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c}{\textbf{Lexical Depth Spearman's Correlation}} & \multicolumn{9}{c}{\textbf{Lexical Distance Spearman's Correlation}} \\
% & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU}
% & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
% \textsc{Distinct} & .813 & .859 & .857 & .838 &  .829 &  &  &  & -
% &  &  &  &  &  &  &  &  &  - \\ \midrule
% \textsc{Mapped} & .811 & .858 & .857 & .839 & .828 &  &  &  &
% &  &  &  &  &  &  &  &  & \\ \midrule
% \textsc{Same} &  .813 & .849 & .850 & .828 &  .799 &  &  & &
% &  &  &  &  &  &  &  &  & \\  \midrule
% \end{tabular}
% \caption{Results on lexical hypernymy structure correlations}
% \label{tab:dependency-depth-results}
% \end{table*}


\begin{table}[!ht]
\centering
\tiny
\begin{tabular}{@{}l|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c}{\textbf{Dependency Distance Spearman's Correlation}}  \\
& \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
\textsc{Distinct} & .813 & .859 & .857 & .856 & .829 & .791 & .839 & .856 & .770 \\
\citet{chi2020finding} & .817 & .859 & - & .807 &  .777 & .812 & .822 & .864 & - \\ \midrule
\textsc{Mapped} & .812 & .857 & .858 & .838 & .831 & .790 & .837 & .854 & .771\\ \midrule
\textsc{Same} & .812 & .851 & .850 & .827 & .789 & .788 & .812 & .850 & .738 \\ 
\citet{chi2020finding} & .806 & .848 & - & .789  &  .717 & .802 & .795 & .853 & - \\ \midrule
\end{tabular}
\caption{Results on dependency structure correlation and Undirected Unlabeled Attachement Score. Compared with \emph{Standard Structural Probes} after \citet{chi2020finding}.}
\label{tab:dependency-distance-results}
\end{table}


\begin{table}[!ht]
\centering
\tiny
\begin{tabular}{@{}l|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c}{\textbf{Dependency Depth Spearman's Correlation}}  \\
& \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
\textsc{Distinct} & .844 & .869 & .869 & .856 & .843 & .824 & .868 & .875 & .796 \\ \midrule
\textsc{Mapped} & .840 & .868 & .866 & .854 & .847 & .821 & .866 & .873 &	.795  \\ \midrule
\textsc{Same} & .837 & .860 & .859 & .844 & .806 & .818 & .835 & 	.870 & 0.766\\ \midrule
\end{tabular}
\caption{Results on dependency structure correlation.}
\label{tab:dependency-depth-results}
\end{table}

\begin{table}[!ht]
\centering
\tiny
\begin{tabular}{@{}l|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c}{\textbf{Dependency Depth Spearman's Correlation}}  \\
& \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
\textsc{Distinct} & .844 & .869 & .869 & .856 & .843 & .824 & .868 & .875 & .796 \\ \midrule
\textsc{Mapped} & .840 & .868 & .866 & .854 & .847 & .821 & .866 & .873 &	.795  \\ \midrule
\textsc{Same} & .837 & .860 & .859 & .844 & .806 & .818 & .835 & 	.870 & 0.766\\ \midrule
\end{tabular}
\caption{Results on dependency structure correlation.}
\label{tab:dependency-depth-results}
\end{table}


\begin{table}[!ht]
\centering
\tiny
\begin{tabular}{@{}l|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c}{\textbf{Lexical Depth Spearman's Correlation}}  \\
& \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
\textsc{Distinct} & .846 & .883 & .779 & .859 & .868 & .778 & .922 & .854 & .848 \\ \midrule
\textsc{Mapped} & .857 & .869 & .789 & .845 & .881 & .805 & .911 & .852 & .865\\ \midrule
\textsc{Same} & .830 & .839 & .748 & .741 & .804 & .780 & .612 & .822 & .830 \\ \midrule
\end{tabular}
\caption{Results on lexical structure correlation.}
\label{tab:lexical-depth-results}
\end{table}


\begin{table}[!ht]
\centering
\tiny
\begin{tabular}{@{}l|ccccccccc@{}}
\toprule
\multicolumn{1}{c|}{\textbf{Approach}} & \multicolumn{9}{c}{\textbf{Lexical Distance Spearman's Correlation}}  \\
& \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
\textsc{Distinct} & .756 & .840 & .644 & .722 & .793 & .646 & .752 & .791 & .676 \\ \midrule
\textsc{Mapped} & .756 & .843 & .619 & .718 & .811 & .667 & .776 & .791 & .675 \\ \midrule
\textsc{Same} & .720 & .820 & .599 & .661 & .791 & .624 & .755 & .779 & .613 \\ \midrule
\end{tabular}
\caption{Results on lexical structure correlation.}
\label{tab:lexical-distance-results}
\end{table}


\begin{table}[!ht]
\centering
\tiny
\begin{tabular}{@{}l|ccccccccc@{}}
\toprule

\textbf{Approach} & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} \\ \midrule
\multicolumn{10}{c}{\textbf{Dependency Distance Spearman's Correlation}} \\ \midrule
\textsc{Distinct} & .813 & .859 & .857 & .856 & .829 & .791 & .839 & .856 & .770 \\
\citet{chi2020finding} & .817 & .859 & - & .807 &  .777 & .812 & .822 & .864 & - \\ \midrule
\textsc{Mapped} & .812 & .857 & .858 & .838 & .831 & .790 & .837 & .854 & .771\\ \midrule
\textsc{Same} & .812 & .851 & .850 & .827 & .789 & .788 & .812 & .850 & .738 \\ 
\citet{chi2020finding} & .806 & .848 & - & .789  &  .717 & .802 & .795 & .853 & - \\ \midrule
\multicolumn{10}{c}{\textbf{Dependency Depth Spearman's Correlation}} \\ \midrule
\textsc{Distinct} & .844 & .869 & .869 & .856 & .843 & .824 & .868 & .875 & .796 \\ \midrule
\textsc{Mapped} & .840 & .868 & .866 & .854 & .847 & .821 & .866 & .873 &	.795  \\ \midrule
\textsc{Same} & .837 & .860 & .859 & .844 & .806 & .818 & .835 & 	.870 & .766\\ \midrule
\multicolumn{10}{c}{\textbf{Lexical Distance Spearman's Correlation}} \\ \midrule
\textsc{Distinct} & .756 & .840 & .644 & .722 & .793 & .646 & .752 & .791 & .676 \\ \midrule
\textsc{Mapped} & .756 & .843 & .619 & .718 & .811 & .667 & .776 & .791 & .675 \\ \midrule
\textsc{Same} & .720 & .820 & .599 & .661 & .791 & .624 & .755 & .779 & .613 \\ \midrule
\multicolumn{10}{c}{\textbf{Lexical Depth Spearman's Correlation}} \\ \midrule
\textsc{Distinct} & .846 & .883 & .779 & .859 & .868 & .778 & .922 & .854 & .848 \\ \midrule
\textsc{Mapped} & .857 & .869 & .789 & .845 & .881 & .805 & .911 & .852 & .865\\ \midrule
\textsc{Same} & .830 & .839 & .748 & .741 & .804 & .780 & .612 & .822 & .830 \\ \midrule
\end{tabular}
\caption{Spearman's Corrrelation between gold and predicted depths and distances.  We probe the representations of 7th layer  for dependency information, and representations of 5th layer  for lexical  information. Correlations for dependency distance are compared with \emph{Standard Structural Probes} reported by \citet{chi2020finding}. Their \textsc{In-Lang} and \textsc{AllLangs} settings correspond to ours  \textsc{Distinct} and \textsc{Same} settings respectively.}
\label{tab:correlation-results}
\end{table}



\begin{figure*}[!ht]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/crossling_corr_dep.pdf}
    \caption{Correlations between probing results for multiple languages, typological similarity to English, and size of mBERT training corpora in specific languages.}
\end{figure*}


\begin{figure}[h]
    \centering
    \begin{subfigure}{0.8\linewidth}
        \resizebox{1.0\linewidth}{!}{\input{figures/heatmap_lex_dep.pgf}}
        \caption{Dependency}
    \end{subfigure}
    \begin{subfigure}{0.8\linewidth}
        \resizebox{1.0\linewidth}{!}{\input{figures/heatmap_lex.pgf}}
        \caption{Lexical}
    \end{subfigure}
    \caption{Pearson's correlation between results from \cref{tab:spearman-results} for each language and two language-specific features: typological similarity to English and number of tokens in Wikipedia.}
    \label{fig:pearson-features}
\end{figure}

\begin{figure*}[h]
    \centering
    \resizebox{0.75\linewidth}{!}{\input{figures/corr_lex.pgf}}
    \caption{lex2}
    \label{fig:lex-features}
\end{figure*}

\begin{figure*}[h]
    \centering
    \resizebox{0.75\linewidth}{!}{\input{figures/corr_dep.pgf}}
    \caption{dep}
    \label{fig:features-correlation}
\end{figure*}

==> sections/table.tex <==
% https://tex.stackexchange.com/a/40603 - only color in table body
\newtoggle{inTableHeader}% Track if still in header of table
\toggletrue{inTableHeader}% Set initial value
% \newcommand*{\StartTableHeader}{\global\toggletrue{inTableHeader}}%
% \newcommand*{\EndTableHeader}{\global\togglefalse{inTableHeader}}%

% % Redefine tabular to initialize \StartTableHeader at start and end
% \let\OldTabular\tabular%
% \let\OldEndTabular\endtabular%
% \renewenvironment{tabular}{\StartTableHeader\OldTabular}{\OldEndTabular\StartTableHeader}%

%  The min, mid and max values
% \newcommand*{\MinNumber}{0} %
% \newcommand*{\MaxNumber}{10}%
% \definecolor{MinAttention}{RGB}{240, 240, 240}

%Apply the gradient macro
\newcommand{\ApplyGradient}[1]{%
  \iftoggle{inTableHeader}{#1}{
        \ifdim #1 pt > \MidNumber pt
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(#1 - \MidNumber)/(\MaxNumber-\MidNumber),100.0),0.00)} %
            %{\setlength{\fboxsep}{0.3pt}\noindent\colorbox{green!\PercentColor!white}{#1}}
        
            \hspace{-0.05em}\colorbox{green!\PercentColor!white}{\ifdim #1 pt < 10 pt \phantom{1}\fi#1}
            %\noindent\colorbox{green!\PercentColor!white}{#1}
        \else
            \pgfmathsetmacro{\PercentColor}{max(min(100.0*(\MidNumber - #1)/(\MidNumber-\MinNumber),100.0),0.00)} %{\setlength{\fboxsep}{0.3pt}\colorbox{red!\PercentColor!white}{#1}}
            \hspace{-0.05em}\colorbox{red!\PercentColor!white}{\ifdim #1 pt < 10 pt \phantom{1}\fi#1}
            %\noindent\colorbox{red!\PercentColor!white}{#1}
        \fi
}}

\newcolumntype{R}{>{\collectcell\ApplyGradient}c<{\endcollectcell}}
\renewcommand{\arraystretch}{0}
\setlength{\fboxsep}{2mm} % box size
\setlength{\tabcolsep}{0pt}

% \begin{table}[t]
%     \begin{minipage}[b]{0.47\textwidth}
%     \definecolor{MaxAttention}{RGB}{43, 130, 23}
%     \footnotesize
%     \begin{tabular}{l*{8}{R}}
%         \rotatebox{90}{}&\rotatebox{90}{ main diagonal}&\rotatebox{90}{ diagonal}&\rotatebox{90}{ vertical}&\rotatebox{90}{ balustrades}&\rotatebox{90}{ rare words}&\rotatebox{90}{ heterogenous}&\rotatebox{90}{ scattered}&\rotatebox{90}{ equal} \EndTableHeader\\
%         L0\,& 6 & 3 & 1 & 0 & 0 & 4 & 2 & 1 \\
%         L1\,& 0 & 0 & 0 & 9 & 0 & 0 & 7 & 0 \\
%         L2\,& 0 & 0 & 0 & 7 & 1 & 0 & 8 & 0 \\
%         L3\,& 0 & 0 & 0 & 6 & 0 & 2 & 8 & 0 \\
%         L4\,& 0 & 0 & 1 & 3 & 0 & 3 & 7 & 0 \\
%         L5~~\,& 0 & 1 & 0 & 8 & 0 & 1 & 5 & 0 \\
%     \end{tabular}
%     \end{minipage}\hfill
%     \begin{minipage}[b]{0.47\textwidth}
%     \definecolor{MaxAttention}{RGB}{50, 126, 171}
%     \footnotesize
%     \begin{tabular}{l*{8}{R}}
%         \rotatebox{90}{}&\rotatebox{90}{ main diagonal}&\rotatebox{90}{ diagonal}&\rotatebox{90}{ vertical}&\rotatebox{90}{ balustrades}&\rotatebox{90}{ rare words}&\rotatebox{90}{ heterogenous}&\rotatebox{90}{ scattered}&\rotatebox{90}{ equal} \EndTableHeader\\
%         L0\, & 0 & 3 & 0 & 0 & 0 & 0 & 9 & 0 \\
%         L1\, & 0 & 2 & 0 & 0 & 0 & 1 & 9 & 0 \\
%         L2\, & 0 & 2 & 0 & 0 & 0 & 0 & 9 & 1 \\
%         L3\, & 0 & 2 & 1 & 0 & 0 & 1 & 8 & 0 \\
%         L4\, & 1 & 2 & 1 & 1 & 0 & 1 & 6 & 0 \\
%         L5\, & 0 & 2 & 0 & 2 & 0 & 3 & 5 & 0 \\
%         L6\, & 0 & 0 & 0 & 1 & 1 & 6 & 4 & 0 \\
%         L7\, & 0 & 0 & 0 & 1 & 0 & 7 & 4 & 0 \\
%         L8\, & 0 & 0 & 2 & 0 & 0 & 4 & 6 & 0 \\
%         L9\, & 0 & 0 & 3 & 2 & 0 & 3 & 4 & 0 \\
%         L10\,& 0 & 0 & 9 & 0 & 0 & 3 & 0 & 0 \\
%         L11~~\,& 0 & 0 & 10& 0 & 0 & 2 & 0 & 0 \\
%     \end{tabular}
%     \end{minipage}
%     \caption[Proportions of the self-attention patterns over layers in \acrshort{nmt} and \acrshort{bert}.]{Proportions of the self-attentions patterns over layers in \acrshort{nmt} (left) and \acrshort{bert} (right).}
%     \label{tab:patterns-in-nmt-and-bert}
% \end{table}
% \renewcommand{\arraystretch}{1}
% \setlength{\tabcolsep}{6pt}
% \setlength{\fboxsep}{3mm} % box size


\begin{table*}[!ht]
\centering
\scriptsize
\begin{tabular}{@{}l|9*{R}|3*{R}@{}}
\toprule
\textbf{Approach} & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} & \multicolumn{3}{c}{\textbf{AVERAGE}} \\
 &  & &  & &  &  &  &  &  & \textbf{I-E} & \textbf{N-I-E} & \textbf{All} \\\midrule
\multicolumn{13}{c}{\textbf{Dependency Distance Spearman's Correlation}} \\ \midrule
\textsc{In-L} & .813 & .859 & .857 & .856 & .829 & .791 & .839 & .856 & .770 & .846 & .817 & .830 \\
\textcolor{blue}{Chi+} & .817 & .859 & - & .807 &  .777 & .812 & .822 & .864 & - & .847 & .805 & .823 \\ \midrule
\toggletrue{inTableHeader}
$\Delta$ \textsc{MapL} &  -.001 &  -.002 &  .000 &  -.017 &  .001 &  -.001 &  -.002 &  -.003 &  .001 &  -.001 &  -.004 &  -.003 \\ \midrule
$\Delta$ \textsc{AllL} &  -.001 &  -.009 &  -.007 &  -.029 &  -.040 &  -.002 &  -.027 &  -.006 &  -.032 &  -.006 &  -.026 &  -.017\\ 
\textcolor{blue}{Chi+} &  -.011 &  -.011 & - &  -.018 &  -.060 &  -.010 &  -.037 &  -.011 & - &  -.011 &  -.031 &  -.023 \\ \midrule
\togglefalse{inTableHeader}
\multicolumn{13}{c}{\textbf{Dependency Depth Spearman's Correlation}} \\ \midrule
\textsc{In-L} & .844 & .869 & .869 & .856 & .843 & .824 & .868 & .875 & .796 & .865 & .837 & .849 \\ %\midrule
\toggletrue{inTableHeader}
$\Delta$ \textsc{MapL} &  -.004 &  -.002 &  -.003 &  -.002 &  .003 &  -.003 &  -.002 &  -.002 &  .000 &  -.003 &  -.001 &  -.002 \\ % \midrule
$\Delta$ \textsc{AllL} &  -.008 &  -.010 &  -.010 &  -.011 &  -.037 &  -.006 &  -.033 &  -.006 &  -.029 &  -.008 &  -.023 &  -.017 \\ \midrule
\togglefalse{inTableHeader}
\multicolumn{13}{c}{\textbf{Lexical Distance Spearman's Correlation}} \\ \midrule
\textsc{In-L} & .756 & .840 & .644 & .722 & .793 & .646 & .752 & .791 & .676 & .758 & .718 & .735 \\ % \midrule
$\Delta$ \textsc{MapL} &  .000 &  .002 &  -.025 &  -.003 &  .018 &  .022 &  .025 &  .000 &  -.001 &  -.006 &  .012 &  .004\\ % \midrule
$\Delta$ \textsc{AllL} &  -.036 &  -.021 &  -.045 &  -.061 &  -.003 &  -.022 &  .004 &  -.012 &  -.062 &  -.029 &  -.029 &  -.029 \\ \midrule
\multicolumn{13}{c}{\textbf{Lexical Depth Spearman's Correlation}} \\ \midrule
\textsc{In-L} & .846 & .883 & .779 & .859 & .868 & .778 & .922 & .854 & .848 & .840 & .855 & .848 \\ % \midrule
\toggletrue{inTableHeader}
$\Delta$ \textsc{MapL} &  .011 &  -.014 &  .010 &  -.014 &  .013 &  .027 &  -.011 &  -.001 &  .017 &  .002 &  .006 &  .004 \\ % \midrule
$\Delta$ \textsc{AllL} &  -.017 &  -.044 &  -.030 &  -.118 &  -.064 &  .002 &  -.311 &  -.031 &  -.017 &  -.031 &  -.102 &  -.070 \\ \midrule
\toggletrue{inTableHeader}
\end{tabular}
\caption{Spearman's correlation between gold and predicted depths and distances.  
%We probe the representations of the 7th layer for dependency information and representations of the 5th layer for lexical information. These layers achieve the highest performance for the respective features. 
The three last columns present averages for Indo-European, Non-Indo-European, and all languages. The evaluation is not zero-shot, we use data in a target language. Correlations for dependency distance are compared with \emph{Standard Structural Probes} reported by \citet{chi-etal-2020-finding}. 
% Their \textsc{In-Lang} and \textsc{AllLangs} settings correspond to ours  \textsc{In-Lang} and \textsc{AllLangs} settings respectively.
}
\label{tab:spearman-results}
\end{table*}


\begin{table*}[!ht]
\setlength{\tabcolsep}{2 pt}
\centering
\small
\begin{tabular}{@{}l|ccccccccc|ccc@{}}
\toprule
\textbf{Approach} & \textbf{EN} & \textbf{ES} & \textbf{SL} & \textbf{ID} & \textbf{ZH} & \textbf{FI} & \textbf{AR} & \textbf{FR} & \textbf{EU} & \multicolumn{3}{c}{\textbf{AVERAGE}} \\
 &  & &  & &  &  &  &  &  & \textbf{I-E} & \textbf{N-I-E} & \textbf{All} \\\midrule
\multicolumn{13}{c}{\textbf{Dependency Distance Spearman's Correlation}} \\ \midrule
\textsc{In-Lang} & .812 & .858 & .857 & .841 & .830 & .788 & .838 & .856 & .769 & .846 & .813 & .828 \\
\textcolor{blue}{Chi et al.} & .817 & .859 & - & .807 &  .777 & .812 & .822 & .864 & - & .847 & .805 & .823 \\ \midrule
$\Delta$ \textsc{MappedL} & \ApplyGradient{.000} & \textbf{\ApplyGradient{-.001}} & \ApplyGradient{.001} & \ApplyGradient{-.003} & \ApplyGradient{.000} & \ApplyGradient{.001} & \ApplyGradient{-.001} & \textbf{\ApplyGradient{-.002}} & \ApplyGradient{.001} & \ApplyGradient{-.001} & \ApplyGradient{.000} & \ApplyGradient{.000} \\ \midrule
$\Delta$ \textsc{AllL} & \ApplyGradient{.000} & \textbf{\ApplyGradient{-.007}} & \textbf{\ApplyGradient{-.006}} & \textbf{\ApplyGradient{-.013}} & \textbf{\ApplyGradient{-.039}} & \ApplyGradient{.000} & \textbf{\ApplyGradient{-.027}} & \textbf{\ApplyGradient{-.006}} & \textbf{\ApplyGradient{-.032}} & \textbf{\ApplyGradient{-.005}} & \textbf{\ApplyGradient{-.022}} & \textbf{\ApplyGradient{-.015}}\\ 
\textcolor{blue}{Chi et al.} & \ApplyGradient{-.011} & \ApplyGradient{-.011} & - & \ApplyGradient{-.018} & \ApplyGradient{-.060} & \ApplyGradient{-.010} & \ApplyGradient{-.037} & \ApplyGradient{-.011} & - & \ApplyGradient{-.011} & \ApplyGradient{-.031} & \ApplyGradient{-.023} \\ \midrule
\multicolumn{13}{c}{\textbf{Dependency Depth Spearman's Correlation}} \\ \midrule
\textsc{In-Lang} & .843 & .868 & .867 & .855 & .844 & .822 & .865 & .877 & .797 & .864 & .837 & .849 \\ %\midrule
$\Delta$ \textsc{MappedL} & \textbf{\ApplyGradient{-.004}} & \textbf{\ApplyGradient{-.003}} & \textbf{\ApplyGradient{-.002}} & \ApplyGradient{-.002} & \ApplyGradient{.000} & \textbf{\ApplyGradient{-.002}} & \ApplyGradient{.001} & \ApplyGradient{-.002} & \ApplyGradient{-.001} & \textbf{\ApplyGradient{-.002}} & \textbf{\ApplyGradient{-.001}} & \textbf{\ApplyGradient{-.002}} \\ % \midrule
$\Delta$ \textsc{AllL} & \textbf{\ApplyGradient{-.006}} & \textbf{\ApplyGradient{-.007}} & \textbf{\ApplyGradient{-.008}} & \textbf{\ApplyGradient{-.011}} & \textbf{\ApplyGradient{-.035}} & \textbf{\ApplyGradient{-.005}} & \textbf{\ApplyGradient{-.031}} & \textbf{\ApplyGradient{-.010}} & \textbf{\ApplyGradient{-.031}} & \textbf{\ApplyGradient{-.008}} & \textbf{\ApplyGradient{-.023}} & \textbf{\ApplyGradient{-.016}} \\ \midrule
\multicolumn{13}{c}{\textbf{Lexical Distance Spearman's Correlation}} \\ \midrule
\textsc{In-Lang} & .756 & .841 & .639 & .719 & .800 & .657 & .733 & .794 & .679 & .757 & .717 & .735 \\ % \midrule
$\Delta$ \textsc{MappedL} & \ApplyGradient{-.003} & \ApplyGradient{.005} & \ApplyGradient{-.011} & \ApplyGradient{-.001} & \textbf{\ApplyGradient{.010}} & \ApplyGradient{.001} & \textbf{\ApplyGradient{.042}} & \ApplyGradient{.001} & \ApplyGradient{-.008} & \ApplyGradient{-.002} & \textbf{\ApplyGradient{.009}} & \ApplyGradient{.004}\\ % \midrule
$\Delta$ \textsc{AllL} & \textbf{\ApplyGradient{-.038}} & \textbf{\ApplyGradient{-.025}} & \textbf{\ApplyGradient{-.042}} & \textbf{\ApplyGradient{-.051}} & \textbf{\ApplyGradient{-.014}} & \textbf{\ApplyGradient{-.043}} & \ApplyGradient{.025} & \textbf{\ApplyGradient{-.013}} & \textbf{\ApplyGradient{-.063}} & \textbf{\ApplyGradient{-.030}} & \textbf{\ApplyGradient{-.029}} & \textbf{\ApplyGradient{-.030}} \\ \midrule
\multicolumn{13}{c}{\textbf{Lexical Depth Spearman's Correlation}} \\ \midrule
\textsc{In-Lang} & .853 & .881 & .779 & .852 & .875 & .784 & .906 & .844 & .842 & .839 & .850 & .845 \\ % \midrule
$\Delta$ \textsc{MappedL} & \ApplyGradient{.004} & \ApplyGradient{-.005} & \textbf{\ApplyGradient{.013}} & \textbf{\ApplyGradient{-.011}} & \ApplyGradient{.006} & \textbf{\ApplyGradient{.023}} & \ApplyGradient{-.024} & \ApplyGradient{.007} & \textbf{\ApplyGradient{.021}} & \textbf{\ApplyGradient{.004}} & \ApplyGradient{.005} & \ApplyGradient{.005} \\ % \midrule
$\Delta$ \textsc{AllL} & \textbf{\ApplyGradient{-.027}} & \textbf{\ApplyGradient{-.048}} & \textbf{\ApplyGradient{-.040}} & \textbf{\ApplyGradient{-.124}} & \textbf{\ApplyGradient{-.068}} & \ApplyGradient{-.006} & \textbf{\ApplyGradient{-.305}} & \textbf{\ApplyGradient{-.032}} & \textbf{\ApplyGradient{-.020}} & \textbf{\ApplyGradient{-.037}} & \textbf{\ApplyGradient{-.103}} & \textbf{\ApplyGradient{-.079}}\\ \midrule
\end{tabular}
\caption{Spearman's correlation between gold and predicted depths and distances.  $\Delta$  denotes the difference from \textsc{In-Lang} results.
%We probe the representations of the 7th layer for dependency information and representations of the 5th layer for lexical information. These layers achieve the highest performance for the respective features. 
The three last columns present averages for \textbf{I}ndo-\textbf{E}uropean, \textbf{N}on-\textbf{I}ndo-\textbf{E}uropean, and all languages. The evaluation is not zero-shot, we use data in a target language. Correlations for dependency distance are compared with \emph{Standard Structural Probes} reported by \citet{chi-etal-2020-finding}. 
% Their \textsc{In-Lang} and \textsc{AllLangs} settings correspond to ours  \textsc{In-Lang} and \textsc{AllLangs} settings respectively.
}
\label{tab:spearman-results2}
\end{table*}
